The Hitchhikers Guide to Rubric Quality Understanding and Enrichment

Rubrics distill notions of expert quality and measure agent performance. However, the quality of rubrics themselves have not been systematically measured and are often left to downstream performance. We import apparatuses from measurement theory built for exactly this: quantitative signals based on the rubric's content, and introduce the RubrIc-Failure Taxonomy (RIFT), of nine possible ways a rubric fails, organized under reliability and content validity. Every mode leaves a distinct signature. To show the signals track failure causally, we seed 720 corruptions, injecting each RIFT mode into clean rubrics at known severity levels. A linear probe over the signals identifies which mode was injected at $75.0\%$ accuracy, beating $56.7\%$ for a frontier model asked to name the failure directly. Surprisingly across GDPval and Terminal-Bench, 10 of 48 expert-authored rubrics weight their criteria backwards, putting more of the score on requirements an expert panel judged less essential. This means a response can fail what matters most and still be graded well. This paper serves as a comprehensive guide on how to understand failure modes in rubrics and create better versions using quality signals, causal experiments, and provides a taxonomy with its rules and examples.

==> archived/abstract_1.tex <==
\section{Abstract}

% Scope and gap
Rubrics distill notions of quality held by domain experts into a single interpretable artifact, enabling automated judging. This makes rubric-based evaluation central to agentic benchmarks and training pipelines. We frame the rubric as a mechanism for distillation: expert judgment is compressed into an artifact that supervises a student model. This framing makes the quality criterion explicit: a rubric is good exactly insofar as the student learns what the expert intended, but that ground-truth test is far too expensive to serve as development-time feedback and no systematic method exists for assessing rubric quality before that cost is paid.
% Quality Signal Ladder
The distillation framing induces a hierarchy of rubric-quality signals ordered by fidelity and cost. At the top sits consequential validity: the performance and learning efficiency of the student model trained with the rubric. One rung down, drawing on education-assessment research, we measure the fidelity of the distillation channel itself with two signals. Reliability asks whether the rubric transmits a consistent signal, and is quantified via inter- and intra-rater reliability and alignment measures. Content validity asks whether the signal carries the construct the teacher intended, and is quantified via a proposed measure inspired by the content validity ratio.
% RIFT Taxonomy and Agent
At the base of the ladder, cheap enough for the inner loop of data development, we introduce RIFT: the RubrIc Failure mode Taxonomy, which systematically characterizes failure modes in rubric composition and design, together with a RIFT review-and-revision agent that uses the taxonomy to identify failure modes and propose revisions. RIFT comprises eight failure modes organized under the same three dimensions: Reliability, Content Validity, and Consequential Validity failures. We develop RIFT using grounded theory, iteratively annotating rubrics drawn from five diverse data sources spanning general instruction following, code generation, creative writing, and expert-level deep research. We then validate each rung of the ladder against the one above it: RIFT agent predictions show <result> correlation with the reliability and content validity signals, which in turn predict downstream training outcomes.
% Open-Benchmark analysis
We then run the RIFT agent on open benchmarks and release the results, finding <result> prevalence of failure modes in expert-authored versus automatically (e.g., contrastively) generated rubrics.
% RL experiments
Finally, we close the loop at the top of the ladder: revising rubrics from RIFT agent critiques improves the mid-tier signals by <result>, and student models trained with revised rubrics achieve <result> higher preference win rates as judged by held-out frontier models demonstrating that failure modes detectable in seconds predict, and their repair improves, training outcomes that cost orders of magnitude more to measure directly.


==> archived/old_background.tex <==
\section{Background}
\label{sec:background}

\subsection*{Rubrics in the era of LLMs}

%What are the main areas of research in the last couple years ab llms and rubs
There has been a rise in research surrounding the appropriate use, evaluation, and understanding of rubrics in the era of LLMs. Broadly, this work falls into three areas: constructing and refining rubrics, applying rubrics to evaluate LLM outputs, and, most recently, assessing the quality of rubrics themselves.

\paragraph{Constructing and refining rubrics.} A growing body of work focuses on building better rubrics and the models that generate or apply them. \citet{liu-etal-2026-openrubrics} curate a large set of prompt-rubric pairs for training rubric-generation and rubric-based reward models. In a similar spirit, \citet{research_rubrics_scale} construct rubric-based datasets targeting specific LLM competencies, including instruction following, research ability, and communication. \citet{shen2026rethinkingrubricgenerationimproving} propose an iterative refinement procedure that decomposes coarse-grained rubrics into finer, more discriminative criteria, improving coverage and separating response quality more sharply. \citet{ding2026adarubrictaskadaptiverubricsreliable} instead generate rubrics adaptively from task descriptions and use them to score agent trajectories step-by-step, producing confidence-weighted reward signals for preference learning. Most closely related to the present work, \citet{dhole2026rubricraginterpretablereliablellm} examine whether LLM-generated rubrics are not only useful for automated downstream evaluation but also interpretable and effective for human users, finding that off-the-shelf LLM-generated rubrics tend to diverge substantially from human-authored ones.

\paragraph{Applying rubrics to evaluation.} A second line of work uses rubrics as the evaluation mechanism itself. \citet{hashemi-etal-2024-llm} introduce a framework in which a manually constructed rubric specifies the dimensions along which a natural language text should be assessed. \citet{wei2025conceptbasedrubricsimprovellm} show that concept-based rubrics can improve LLM evaluation performance on STEM student-response datasets of varying label quality, narrowing the gap between LLM-based assessment and smaller supervised models, and further use these rubrics to generate synthetic training data for lightweight supervised evaluators.

%hook 
\paragraph{Assessing rubric quality.} A third and much more nascent line of work asks a different question: not how to build or apply a rubric, but whether a given rubric is itself \emph{good}. Historically, rubric quality has been inferred only indirectly, through downstream signals such as reinforcement-learning outcomes or judge--human agreement, which conflates the quality of the rubric with the behavior of whichever judge applies it. \citet{arabzadeh-etal-2024-assessing} take an early step toward isolating rubric quality directly, introducing a verifier agent that checks whether evaluation criteria are essential, robust, informative, and discriminative, using stability checks and adversarial random-deletion tests to prune redundant or non-discriminative criteria. \citet{pan2026rubricevalrubriclevelmetaevaluation} argue that response-level meta-evaluation is insufficient and introduce a rubric-level meta-evaluation benchmark, showing that even strong LLM judges struggle to apply rubric-level criteria reliably and that explicit reasoning over rubric criteria reduces inter-judge variance. \citet{siro2026learningjudgellms} evaluate the semantic coherence, scoring reliability, and human-alignment of LLM-generated rubric criteria across several NLG benchmarks, finding that closed-source models produce more reliable and cross-model-consistent rubrics than open-weight models, and that reliability degrades further in factual, knowledge-intensive settings. \citet{hong2026canllmswrite} conduct a meta-evaluation of LLM-generated rubrics for scientific paper reproduction, assessing rubric quality both intrinsically, via similarity to human-authored rubrics, and extrinsically, via alignment with ground-truth scores, and find that generated rubrics are systematically over-specific, code-centric, and biased toward high scores relative to human-authored ones. \citet{roy2026premisepolicyrubricsmeasurement} treat rubrics as measurement specifications and propose auditing them directly along four axes---structural adequacy, reliability, preference fit, and adversarial robustness---explicitly cautioning that agreement between judges is not the same as validity, and that fitting human preferences is not the same as robustness to gaming. 

%commenting this out since we are citing this as a contribution
% \citet{qi2026riftrubricfailuremodetaxonomy} develop a grounded taxonomy of rubric failure modes spanning reliability, content-validity, and consequential-validity failures, together with automated diagnostics that detect these failure modes directly from a rubric's structure rather than from downstream judge behavior.

%reel
\subsection*{The history and design of rubrics: lessons outside CS}

Long before rubrics became a tool for LLM evaluation, they were studied extensively in educational assessment, where a substantial literature addresses what makes a rubric valid and effective. One key distinction is between analytic and holistic rubrics: analytic rubrics assess criteria one at a time and are generally better suited to giving students formative feedback, while holistic rubrics collapse all criteria into a single overall judgment, making them faster to apply but less informative when feedback is the goal \citep{brookhart2018appropriate}.

A second, related body of work addresses instrument validity more broadly, since a rubric is fundamentally a measurement instrument. \citet{ghauri2005research} define validity in terms of how well a collected sample covers the domain under investigation, and \citet{field2005discovering} frame the validity of a rubric specifically as the extent to which it measures what it is intended to measure. \citet{taherdoost2016validity} decomposes validity into several distinct types: \emph{criterion validity}, concerned with how strongly a measure relates to an outcome of interest; \emph{face validity}, a largely subjective judgment that is often treated as the weakest and least essential form of validity; \emph{content validity}, defined by \citet{straub2004validation} as the degree to which the items of an instrument reflect the full content universe to which the instrument is meant to generalize; and \emph{construct validity}. Content validity in particular has a well-established quantitative treatment, dating to \citet{lawshe1975quantitative}, who proposed a method for numerically estimating the degree to which a panel of judges agrees that an item is essential to the construct being measured.

Beyond defining these validity types, researchers have also built concrete tools for assessing them. \citet{brookhart2015quality} examine what makes descriptive rubrics effective in practice, while \citet{montes2023design} propose a decision-support system for establishing consensus content validity of a questionnaire, using a Delphi-based method extended with two-tuple fuzzy linguistic representations to aggregate expert judgments.


%sinker
\subsection*{The main takeaways}

Taken together, this literature suggests that the NLP community's recent enthusiasm for rubrics as an evaluation tool has largely proceeded without engaging the substantial prior work on rubric and instrument validity from educational measurement and the social sciences. While a handful of very recent efforts have begun to isolate and diagnose rubric quality directly, this work remains fragmented in its terminology and criteria. In this paper we bridge this gap and provide a thorough analysis of rubrics by grounding the analytical methods in its own domain and literature. We show numeric signals and the effects of rubric changes on these numbers so researchers can be wary and alert of rubric quality early. We also generate AI written rubrics and study these features to see whether AI can reliably generate quality rubrics. 

==> archived/old_quality_signals.tex <==


\section{Quality Signals and Measures}
\label{sec:quality_signals}
% cad 09/02: Overall I feel we can organize and tighten by scoping this section to the contribution of the definition of the quality signals and an intuitive description of how they should be interpretted. Then move any experimental parameters and content or more extensive related work discussion to respective sections.

Rubric and checklist-based grading has become the default instrument for evaluating open-ended LLM behavior. 
% cad 09/02: These are nice but I feel we can be tighter with intro / motivation here and move to related work section. 
From physician-authored clinical rubrics \citep{arora2025healthbench} and expert authored research-replication tasks \citep{starace2025paperbench} to rubric-derived reward signals \citep{gunjal2025rubrics} and generated checklists \citep{cook2024ticking, qin2024infobench}. 
% cad 09/02: Similar to above, i feel this could fit into related work and should have a more direct paraphrase or quote to prove that work has established validation via "\emph{grader's} fidelity to a rubric".
Yet this line of work has mostly validated the \emph{grader's} fidelity to a rubric, not the rubric's fidelity to the task. 
We measure the latter. 
% cad 09/02: notation needs introduction. what is c_i and w_i? and also there looks to be an error: "($M\!\in\![6,31]" no closed paren and why start at 6?
Our corpus is $T{=}60$ agentic-benchmark tasks: 30 derived from GDPval \citep{patwardhan2025gdpval} and 30 from Terminal-Bench \citep{merrill2026terminalbench}, each with a human-authored rubric of weighted items $\{(c_i, w_i)\}_{i=1}^{M}$ ($M\!\in\![6,31]$; 
% cad 09/02: this feels different from M\!\in\![6,31], why do they live in same paren? that is index of c and w while this next phrase is referencing weight bounds in text rather than math.
Terminal-Bench rubrics include negatively weighted penalty items). 
% cad 09/02: what is "item" refering to? 
Throughout, item scoring mass is $s_i = |w_i| / \sum_k |w_k|$. 
% cad 09/02: Do we only use GPT 5.5? that may raise reviewer concerns. 
% cad 09/02: GPT 5.5 feels like an experimental hyperparam not something we need to define the quality signals.
% cad 09/02: Personas seems significant to the definition of these quality signals. More details should be added and also persona prompts added to the appendix/prompts.tex.  
% cad 09/02: Reference to signals as "three lenses" started to confuse me. Can we be consistent and call them quality signals/signals/metrics(maybe) throughout.
All three lenses are instantiated with GPT-5.5 panels whose personas are generated per task \emph{from the task instruction alone} and \textbf{never from the rubric under evaluation} to avoid circularity; where a lens contrasts human against AI-generated rubrics, the AI rubric is generated from the same instruction with the same item count.
Prompts, configurations, and per-item outputs will be released with our code in a camera ready version. 

\subsection{Content validity ratio}
\label{sec:exp-cvr}
% cad 09/02: Can we align on terminology for rubric structure and clarify before this? Some proposal: \emph{rubrics} are collections of \emph{criteria} each with a corresponding numerical \emph{weight} representing its importance. Item here I am reading as being a "criterion".
% cad 09/02: I feel like the "five-decade quantitative tradition" should be something from five-decades ago, like lawshe1975quantitative rather than almanasreh2019evaluation.
Content validity, which measures whether each item belongs on the whole rubric instrument, has a five-decade quantitative tradition \citep{almanasreh2019evaluation}. 
% cad 09/02: Should we introduce (CVR) acronym here?
Its classical statistic is Lawshe's content validity ratio \citep{lawshe1975quantitative}: a panel of $N$ experts labels each item \emph{essential} or not, and
% cad 09/02: \mathrm{CVR}_i needs more setup. Maybe in previous sentence something like "...or not, and the content validity ration for a criterion with index $i$ is:"
\begin{equation}
    \mathrm{CVR}_i \;=\; \frac{n_i^{e} - N/2}{N/2} \;\in\; [-1, 1],
    \label{eq:cvr}
\end{equation}
where $n_i^{e}$ is the number of essential votes for item $i$; we report a rubric's mean CVR, alongside the adjacent content-validity-index tradition's caution to state the aggregation explicitly \citep{polit2006content}. 
We instantiate the panel with $N{=}5$ task-adapted LLM personas \footnote{\citet{lawshe1975quantitative} recommends at least five experts},
% cad 09/02: Similar to above this feels more important than footnote, it is part of our primary contribution. 
\footnote{
    A task adapted LLM persona is a set of human personas that are directly relevant to the domain at hand. 
    So for a task on contract law the five personas would be a mix of contract experts, legal experts, and contract law experts.
} 
% cad 09/02: Is there something from these citations to back up how we define the personas? 
We rationalize using LLM annotators following \citep{gilardi2023chatgpt}'s work stating they match or exceed non-expert human raters on structured labeling and \citep{verga2024replacing}'s work showing that task-adapted diverse panels reduce single-judge bias, and persona conditioning yields genuinely differentiated, expertise-sensitive raters rather than five draws from one distribution \citep{argyle2023outofone, salewski2023incontext}.


%MAYBE WE need to include this in a rebuttal but it seems premature for the original submission
% Two honest
% limitations follow from the psychometric literature. First, at $N{=}5$ the CVR
% is coarsely discrete ($\mathrm{CVR}_i \in \{-1,-0.6,\dots,1\}$) and the exact
% critical value is $1.0$---unanimity---once Lawshe's original table is
% corrected \citep{wilson2012recalculation, ayre2014critical,
% romero2023lawshereview}; we therefore treat mean CVR as a descriptive
% agreement statistic, not a significance-tested retention rule. Second,
% persona panels compress the between-rater variance that CVR is designed to
% exploit \citep{bisbee2024synthetic}, so our scores are a reproducible screen,
% not a substitute for a convened human panel.

\subsection{Domain mapping}
\label{sec:exp-domain}

% cad 09/02: Similar to previous section, I feel this introduction/motivation paragraph  can be tightened and this content brought to related work and then emphasis here is on our contribution of what we did to adapt this to rubrics for AI.
\citet{fives2013tos}'s work on classroom assessment protocol development and the blueprint-then-expert-review steps of the MEASURE protocol \citep{kalkbrenner2021measure} support that instrument-development protocols require an explicit content plan before items are judged. 
Validity theory supplies the two questions such a plan must answer, distinguishing content \emph{relevance} (does an item belong to the domain?) from content \emph{representativeness}(does the item set cover the domain in the right proportions?) \citep{messick1989validity, haynes1995content, sireci1998content}.
Alignment methodology turns these into gradeable criteria with a thresholds such as Webb's balance-of-representation criterion \citep{webb1997criteria, webb2007alignment} and Porter's scalar alignment index \citep{porter2002content}. 
While a fourth tradition places items in a domain \emph{geometry} via SME ratings and multidimensional scaling \citep{sireci1992analyzing, sireci1995smes}, with radial distance-from-center itself long recognized as measurement-bearing structure in the radex \citep{guttman1954radex, marshalek1983radex}. 
To our knowledge no existing rubric-validation framework combines these elements; our domain mapping is a new hybrid that automates all four. 
We combine these elements and provide an automated way to view rubric validity at a group view. 
The previous section \ref{sec:exp-cvr} evaluates rubrics at the item-importance level, while here we evaluate at the distribution level. 

% cad 09/02: concentric relevance rings sounds a bit unnatural, can we call it relevance levels or something simpler?
For each task, an LLM generates from the instruction a domain map of five concentric relevance rings around the task's domain 
% cad 09/02: is centerviz a typo?
centerviz \textsc{core}, \textsc{adjacent}, \textsc{background}, \textsc{general}, and \textsc{irrelevant}. 

A classifier call assigns every rubric item to exactly one ring. 
% cad 09/02: "The resulting ring shares $p_r$" does this mean $p_r$ is the set of classifications for "ring" 'r'?
% cad 09/02: Are the "...human and AI rubrics" introduced yet? This feels like experimental setup and points rather than this section introducing definitions of quality signals. 
The resulting ring shares $p_r$ are compared against blueprint-style coverage targets ($p_{\textsc{core}}\!\geq\!.50$, $p_{\textsc{adj}}\!\geq\!.20$, $p_{\textsc{bg}}\!\geq\!.20$, $p_{\textsc{gen}}\!\geq\!.10$, and any \textsc{irrelevant} item flagged), yielding a five-bit coverage vector and per-ring distributions; the same per-task map and classifier are applied to the human and AI rubrics. 

\subsection{Cross-lens expert judging}
\label{sec:exp-crosslens}

The third lens ports the classical item--objective validation apparatus to LLM rubrics. 
Following the structured-elicitation tradition \citep{dalkey1963experimental}, a panel of $E{=}5$ expert personas independently proposes task objectives from the instruction; proposals are consolidated into a canonical blueprint of $J$ objectives with normalized target weights $W_j$ and centrality tiers, mirroring practice-analysis methods that derive numeric blueprint weights from expert judgment \citep{raymond2001job, lawshe1975quantitative}. 
An LLM judge \citep{zheng2023judging} scores the panel's agreement and the objectives' verifiability. 
Every expert then rates every item's relevance to every objective on a 0--3 scale---the index-of-item--objective-congruence procedure \citep{rovinelli1976content}, in its multidimensional form \citep{turner2003indexes}---giving $\bar{R}_{ij} \in [0,1]$ after averaging over experts and rescaling. 
% cad 09/02: Perhaps a table or some structure for these definitions? Then itd be nice to give reader an interpretation.
Classical construct threats then fall out as computable quantities \citep{messick1989validity}: \emph{item relevance} $\frac{1}{M}\sum_i \max_j \bar{R}_{ij}$ and \emph{weighted relevance} $\frac{1}{M}\sum_i \sum_j W_j \bar{R}_{ij}$; \emph{representativeness} $= 1 - \mathrm{JSD}(W \,\|\, A)$, where $A_j \propto \sum_i s_i \bar{R}_{ij}$ is realized coverage and JSD is the base-2 Jensen--Shannon divergence, bounded in $[0,1]$ \citep{lin1991divergence}, so its complement quantifies construct \emph{under}representation; \emph{contamination}, the $s_i$-weighted share of relevance mass on background- and irrelevant-tier objectives, quantifies construct-\emph{irrelevant} variance \citep{haladyna2004construct}; and \emph{redundancy}, the mean cosine similarity among item pairs whose objective-relevance vectors exceed a duplicate threshold of $0.8$ (zero if none), penalizes duplicated content that inflates apparent information without adding any \citep{boyle1991item, yen1993scaling}. 
% cad 09/02: what is "gold criterion"?
% cad 09/02: Is this a separate quality signal? We should give it an interpretable lable if so to align with experimental results.
Because rubric quality admits no gold criterion, we follow the nomological-net logic of construct validation \citep{cronbach1955construct} and close the net with a discriminant test \citep{campbell1959convergent}: expert-written positive controls, adjacent-but-wrong-domain near negatives, generic quality items, and far negatives (three per class) are scored on the same scale, and we report the margins separating candidate items from each control class---a valid rubric must not merely score its own items highly but separate them from plausible impostors, a check aimed squarely at the known biases of LLM judges \citep{zheng2023judging, salewski2023incontext}.

\subsection{Weight calibration}
\label{sec:exp-weight}
% cad 09/02: Lets make sure 'rubric's weight vector $w$' is defined in setup notation earlier.
None of the preceding lenses examine the rubric's weight vector $w$ itself: content validity asks whether item $i$ belongs, domain mapping asks where it sits, and cross-lens judging asks how much of it is relevant --- but a rubric that gets every item right can still misrepresent the construct if $w$ allocates score mass to the wrong items. 
This is a validity concern in its own right: practice-analysis methods derive numeric blueprint weights directly from expert judgment \citep{raymond2001job, lawshe1975quantitative}, so a rubric's weights are themselves a testable claim about relative importance, not merely a scoring convenience. 
% cad 09/02: $N{=}5$ feels like this is an experimental hyperparameter. Lets reserve for that section.
We introduce three statistics that test this claim against the same $N{=}5$ panel used for $\mathrm{CVR}_i$ (Eq.~\ref{eq:cvr}), so no additional annotation is required.

\emph{Ordering calibration} asks whether $|w_i|$ ranks items the way the
panel does, via the Spearman rank correlation
\begin{align}
    \rho_{\mathrm{ord}} = \mathrm{Spearman}\big(\{|w_i|\}_{i=1}^M,
    \{\mathrm{CVR}_i\}_{i=1}^M\big) \in [-1, 1],
    \label{eq:ordcvi}
\end{align}
undefined, by convention, when either vector is constant (e.g.\ every item rated essential). 
$\rho_{\mathrm{ord}} \approx 1$ indicates weights track panel necessity; $\rho_{\mathrm{ord}} < 0$ indicates weights are \emph{anti-calibrated} --- the rubric would score a response higher for satisfying \emph{less} essential items over more essential ones.

Let $\mathcal{C} = \{i : \mathrm{CVR}_i > 0\}$ denote the panel-endorsed \emph{core} items (majority essential). 
\emph{Failure score retention} (FSR) is the worst-case score fraction a response retains after failing exactly one core item and satisfying every other:
\begin{align}
    \mathrm{FSR} = \max_{i \in \mathcal{C}} \left(1 - \frac{|w_i|}
    {\textstyle\sum_{k: w_k > 0} w_k - \sum_{k: w_k < 0} w_k}\right),
    \label{eq:fsr}
\end{align}
which reduces to $1 - \min_{i \in \mathcal{C}} s_i$ under all-positive weights. 
High FSR flags rubrics where a core failure is cheaply compensated by unrelated credit elsewhere. 
Relatedly, \emph{core weight share} $\sum_{i \in \mathcal{C}} s_i$ reports what fraction of total scoring mass the panel-endorsed items command at all.

% cad 09/02: To organize discussion, lets move this to 5.1 or 6. I feel this section should just be the abstract quality signal definitions.
Because $w$ is a numeric vector rather than free text, it additionally admits a \emph{deterministic} corruption operator for the causal injection study in Experiment 3 --- reallocating a $\rho$ fraction of scoring mass from $\mathcal{C}$ to non-core items --- unlike the LLM-authored rewrites required for the text-based failure modes.


==> sections/future_work.tex <==
In this paper, we develop and validate intrinsic signals for diagnosing RIFT failure modes in rubrics. While our results establish that controlled RIFT failures leave identifiable signatures in these signals, they do not yet show whether intrinsic rubric quality translates into downstream results. A natural next step is therefore to validate RIFT through reinforcement learning, where rubric quality can be tested through its effect on the behavior of trained models. One direct setting is to train and compare models using reward signals derived both from clean rubrics and corrupted rubrics containing controlled RIFT failures.

Another important direction is to evaluate RIFT on naturally occurring rubric failures. Our causal experiments isolate individual failure modes through controlled interventions allowing us to identify the signals associated with each mode. Real-world rubrics may instead contain subtler defects and multiple interacting failure modes. Studying these failures in practice would clarify how naturally occurring defects fit within the RIFT taxonomy and whether their signal patterns align with the controlled interventions studied here.

Finally, the current weighting analysis measures the allocation of absolute weight magnitude across criteria. Future work should model the distinct roles of positive rewards, negative penalties, hard gates, and other non-standard scoring rules. Evaluating these richer scoring semantics would allow the framework to test whether a rubric’s full scoring procedure, rather than only its allocation of additive weight, reflects the intended priorities of the task.

==> sections/limitations.tex <==
% I dumped a broad set of potential limitations below
% We can decide which of these we want to keep or not.

\paragraph{Limited rubric coverage:}
We evaluate 60 human-authored rubrics from two long-form agentic benchmarks, so the findings may not generalize to other task domains, rubric populations, or scoring structures.

Our evaluation uses 30 rubrics each from GDPVal and Terminal-Bench, both of which assess long-form agentic tasks. The resulting corpus is a useful starting point, but the observed signals and failure-mode signatures may not transfer beyond this setting. In addition, our corpus primarily reflects criterion-based rubrics whose scores can be analyzed as an additive allocation across items. Although some evaluated rubrics include negatively weighted penalty items, our current weight signals use absolute weight magnitude and do not distinguish the semantic role of negative versus positive weights or more complex scoring rules generally.

\paragraph{Controlled corruptions are not naturally occurring failures:}
We validate the framework using intentionally corrupted rubrics, which may not capture the messier failures that arise in practice.

Our causal experiments provide a controlled test of whether the proposed signals respond when a specified failure mode is introduced into an otherwise fixed rubric. These interventions do not fully capture naturally occurring rubric defects which may be more subtle and involve multiple interacting failure modes. The resulting signals may therefore not apply as directly in messier real-world settings.

\paragraph{Connection to downstream outcomes:}
This paper studies intrinsic rubric quality, but does not yet show how its signals or RIFT failures affect evaluation or training outcomes.

Our analysis tests whether the proposed signals respond when a specified failure mode is introduced into a rubric but does not measure whether these signals predict the outcomes that ultimately matter in use such as downstream training behavior. The results therefore provide evidence that the signals correlate to RIFT failures, but do not yet establish that a rubric with stronger signal values will produce better downstream evaluations or training outcomes. In addition, the practical effects of failure modes such as reliability and hackability are not directly tested, so we do not yet know whether they lead to lower agreement between graders or exploitable scoring behavior in practice.

\paragraph{Reliance on LLM-based panels:}
Our framework relies on GPT-5.5 to generate task-specific expert panels which may introduce shared-model biases and make comprehensive rubric audits costly.

Our measures depend on LLM-generated personas and judgments. While using different personas is intended to produce a diverse panel, each panelist is instantiated by the same underlying model and may therefore share blind spots, especially on specialized or ambiguous tasks. These shared biases may affect the panel’s judgments and therefore the resulting signal values. In addition, the framework requires multiple LLM calls to construct and apply the panel for each rubric making the cost of a comprehensive audit potentially high.

\paragraph{Incomplete failure-mode coverage:}
The current taxonomy and signal set do not capture every way a rubric can fail, and some RIFT failures are uninformative. 

The current framework evaluates nine RIFT failure modes, but neither the taxonomy nor the signal set is exhaustive. In our experiments, ungrounded verification is only weakly detected, two signals do not respond to any of the tested failure modes, and ordering calibration is undefined when the panel rates all criteria as essential. These results show that the framework should be used as a diagnostic aid for identifying potential issues, rather than as a certificate that a rubric is free of failure.
